From Words to Actions: Unveiling the Theoretical Underpinnings of LLM-Driven Autonomous Systems

In this work, from a theoretical lens, we aim to understand why large language model (LLM) empowered agents are able to solve decision-making problems in the physical world. To this end, consider a hierarchical reinforcement learning (RL) model where the LLM Planner and the Actor perform high-level task planning and low-level execution, respectively. Under this model, the LLM Planner navigates a partially observable Markov decision process (POMDP) by iteratively generating language-based subgoals via prompting. Under proper assumptions on the pretraining data, we prove that the pretrained LLM Planner effectively performs Bayesian aggregated imitation learning (BAIL) through in-context learning. Additionally, we highlight the necessity for exploration beyond the subgoals derived from BAIL by proving that naively executing the subgoals returned by LLM leads to a linear regret. As a remedy, we introduce an $\epsilon$-greedy exploration strategy to BAIL, which is proven to incur sublinear regret when the pretraining error is small. Finally, we extend our theoretical framework to include scenarios where the LLM Planner serves as a world model for inferring the transition model of the environment and to multi-agent settings, enabling coordination among multiple Actors.

==> tex/main/conclusion.tex <==
\normalsize
\section{Conclusion}
In this work, we embedded the LLM agent into a hierarchical RL framework named PAR system. At the high level, the LLM planner decomposed the user-specified task into subgoals, and at the low level, actor(s) translated the linguistic subgoals into physical realizations. The actor also provided feedbacks for augmenting the planning process through a trained reporter. 
In the context of a perfectly pretrained scenario, we elucidated the Bayesian Adaptive Imitation Learning (BAIL) nature of the LLM-aided planning pipeline. Our findings demonstrated that LLMs comprehend the environment through Bayesian inference on historical data and make decisions following expert policy learned during pretraining. 
In practical scenarios, we examined how training errors from both the LLM and the reporter contribute to the ICL error. 
To navigate the exploration-exploitation tradeoff, we introduced an $\epsilon$-greedy exploration strategy, achieving $\sqrt{T}$-regret for both ideal and practical settings.
Finally, we extend our theoretical framework to include scenarios where the LLM Planner serves as a world model for inferring the transition model of the environment and to multi-agent settings, enabling coordination among multiple Actors.

